Analysis of Knowledge Transfer in Kernel Regime

Knowledge transfer is shown to be a very successful technique for training neural classifiers: together with the ground truth data, it uses the "privileged information" (PI) obtained by a "teacher" network to train a "student" network. It has been observed that classifiers learn much faster and more reliably via knowledge transfer. However, there has been little or no theoretical analysis of this phenomenon. To bridge this gap, we propose to approach the problem of knowledge transfer by regularizing the fit between the teacher and the student with PI provided by the teacher. Using tools from dynamical systems theory, we show that when the student is an extremely wide two layer network, we can analyze it in the kernel regime and show that it is able to interpolate between PI and the given data. This characterization sheds new light on the relation between the training error and capacity of the student relative to the teacher. Another contribution of the paper is a quantitative statement on the convergence of student network. We prove that the teacher reduces the number of required iterations for a student to learn, and consequently improves the generalization power of the student. We give corresponding experimental analysis that validates the theoretical results and yield additional insights.

==> experiments.tex <==

\begin{figure*}[ht!]
    \centering
    \subfigure[MNIST training loss]
    {
        \includegraphics[width=0.32\textwidth]{images/loss_mnist}
        \label{fig:train_loss_mnist}
    }
    \subfigure[CIFAR-10 training loss]
    {
        \includegraphics[width=0.32\textwidth]{images/loss_cifar}
        \label{fig:train_loss_cifar}
    }
    \subfigure[CIFAR-10 projections]
    {
        \includegraphics[width=0.32\textwidth]{images/eigs_cifar_new}
        \label{fig:train_projections_loss_cifar}
    }
    \caption{Performance on MNIST and CIFAR-10 training datasets. We observe that the different kernels yield faster convergence of the loss function on training data compared to non-kernel variant. Figure \ref{fig:train_projections_loss_cifar} demonstrates alignment of top eigenvalues and the projections of true labels on corresponding eigenvectors.}
    \label{fig:train_loss}
\end{figure*} 


%\subsection{Setup}
We perform our numerical analysis on two commonly-used datasets for validating deep neural models, i.e., MNIST and CIFAIR-10. These datasets are used for the experiments in \cite{Arora19}. As in their work we only look at the first two classes and set the label $y_i=+1$ if image $i$ belongs to the first class and $y_i=-1$ if it belongs to the second class. The images are normalized such that $||\bm x_i||_2=1$. This is also done for the different kernel embeddings such that $||\bm \phi(\bm x_i)||_2=1$.
\label{data}

The weights in equation \eqref{eq:model} are initialized as follows:
\begin{equation}
    \bm w_i \sim \mathcal{N}(0, k^2 \bm{\mathcal{I}}), \, a_r \sim \text{Unif}(\{-1,1\}), \forall r \in [m].
\end{equation}

We then use the following loss function to  train the model to predict the image labels.
\begin{equation}
\Phi(\mathbf{W}, \mathbf{a}) = 1/2 \sum_{(i=1)}^n(y_i- f_{\mathbf{W},\mathbf{a}}(\mathbf{x}))^2
\end{equation}

For optimization, we use (full batch) gradient descent with the learning rate $\eta$. In our experiments we set $k=10^{-2}, \eta=2 \times 10^{-4}$ similar to \cite{Arora19}.

\subsection{Gaussian kernel method}
We first use the Gaussian kernel 
\begin{equation}
    \mathcal{K}(\bm x_i, \bm x_j) := \exp\left(- \gamma \|\bm x_i - \bm x_j\|^2\right).
\end{equation}
The corresponding embedding is infinite dimensional, hence we consider the fast approximations to the kernel given by \emph{random Fourier features} (RFF) \cite{RR07}. The idea of random Fourier features is to construct an explicit feature map which is of a dimension much lower than the number of observations, but  the resulting inner product approximates the desired kernel function. We use $\gamma=1$ in all our experiments.

\subsubsection{Optimization}
We first investigate the use of Gaussian kernels for a more efficient optimization of the loss function on the training data. Figures \ref{fig:train_loss_mnist} and \ref{fig:train_loss_cifar} show the training loss at different steps respectively on MNIST and CIFAR-10 datasets. We consistently observe that the different Gaussian kernels (specified by various dimensions of the kernel) yields faster convergence of the optimization procedure on both datasets. MNIST is a simple dataset which gives incredibly high score almost immediately, as shown by the train loss (Figure \ref{fig:train_loss_mnist}) and by the accuracy on the test data (the table in Figure \ref{tab:testacc_mnist}) thus we will focus our analysis on the CIFAR-10 dataset. Similar to the setup in \cite{Arora19}, in Figure \ref{fig:train_projections_loss_cifar}, for different methods, we plot the projections of the true class labels on the eigenvectors (i.e., the projections $\{(\mathbf v_i^{T}\mathbf y)^2\}_{i=0}^{n-1}$). For better visualization, we plot the cumulative forms
\begin{equation}
f_i = \sum_{j=0}^i(\mathbf v_j^{T}\mathbf y)^2
\label{eq:overlap_measure}
\end{equation}

which are normalized such that $\sum_{i=0}^{n-1}(\mathbf v_i^{T}\mathbf y)^2=1$.

The results show that using kernels yield a better alignment of the projections with the top eigenvalues, leading to faster convergences. In other words, with kernels, we attain larger $(\mathbf v_i^{T}\mathbf y)^2$'s for top eigenvalues. 
%\begin{figure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{images/eigs2_mnist}
%    \caption{MNIST Projection is not cumsum($|v^T_iy|$)}
%    \label{fig:my_label}
%\end{figure}
%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{images/eigs2_cifar}
%    \caption{CIFAR-10 Projection is not cumsum($|v^T_iy|$)}
%    \label{fig:my_label}
%\end{figure}

\subsubsection{Generalization}
We next investigate the generalization performance of the Gaussian kernel method by analyzing the values of equations \eqref{eq:gen} and \eqref{eq:gen_kernel}. Table \ref{tab:yHy} shows this quantity for different settings and kernels respectively on MNIST and CIFAR-10 datasets. We observe that in both datasets with several kernels we obtain a lower theoretical upper bound on the generalization error compared to the no-kernel case. It is clear that the bound improves as the dimension of the representations increases but also that the generalization bound seems quite sensitive to values of $\gamma$.

\begin{table}[t!]
    %\vspace{-2mm}
    \centering
    \caption{Quantification of $\mathbf y^T(\mathbf H^\infty)^{-1}\mathbf y$ (or $\mathbf y^T(\mathbf H(\mathcal{K})^\infty)^{-1}\mathbf y$ for Gaussian kernels  in different experimental settings. For both datasets, most of the Gaussian kernels yield smaller upper bounds on generalization error.}
    \begin{tabular}{l l l  r}
    
    \toprule
    $\gamma$ & Dimension  & MNIST & CIFAR-10 \\
     \midrule
          0.01 & $\infty$ & 6235 & 271604 \\
          0.1 & $\infty$ & 1519 & 71066\\
          1 & $\infty$ & 442 & 16680\\
          10 & $\infty$ & 9841   & 1236\\
          \midrule
          1 & 500 & 790  & 55501\\
          1 & 1000 & 679 & 51487 \\
          1 & 3072 & 534 & 47471\\
          1 & 10000 & 478 & 44630 \\
          \multicolumn{2}{l}{No kernel} &  789  &  74670\\
        \bottomrule
    \end{tabular}
    \label{tab:yHy}
    %\vspace{-5mm}
\end{table}


\begin{figure}[htb!]
    \centering
    %\hspace{-5mm}
    \subfigure[Test error on CIFAR-10 data.]
    {
        \includegraphics[width=0.9\columnwidth]{images/testloss_cifar}
        \label{fig:testloss_cifar}
    }
    %\hspace{-7mm}
    \subfigure[Test accuracy on CIFAR-10 data.]
    {
        \includegraphics[width=0.9\columnwidth]{images/testacc_cifar}
        \label{fig:testacc_cifar}
    }
    %\hspace{-6.5mm}
%    \subfigure[Test accuracy on MNIST data.]
%    {
%        \includegraphics[width=0.4\textwidth]{images/test_acc_mnist_table}
%        \label{fig:testacc_mnist}
%    }
    \caption{Experimental test errors and accuracy on the test set at the different steps of the Gradient Descent optimization algorithm for CIFAR-10 dataset.
%    For MNIST, we report the accuracy at the different steps of the Gradient Descent optimization where performance is very good with different steps and parameters.}
}
    %
    \label{fig:test_accuracy}
    %\vspace{-2mm}
\end{figure}
%
\begin{figure*}[htb!]
    \centering
    \subfigure[Training loss.]
    {
        \includegraphics[width=0.32\textwidth]{images/loss_cifar_twolayer_full}
        \label{fig:trainloss_neural}
    }
    \subfigure[Test loss]
    {
        \includegraphics[width=0.32\textwidth]{images/testloss_cifar_twolayer_full}
        \label{fig:testloss_neural}
    }
    \subfigure[Projections]
    {
        \includegraphics[width=0.32\textwidth]{images/eigs_twolayer_other_new}
        \label{fig:train_projections_loss_neural}
    }
    \caption{Experimental train and test errors at the different steps of Gradient Descent as well as eigenvector projections for the CIFAR-10 dataset. For the model pre-trained with the same labels, the training loss and projections are calculated based on the unseen subset of training data. We observe that neural embeddings improve the convergence, generalization and the alignment of eigenvector projections.}
    \label{fig:neural_kernel}
    %\vspace{-2mm}
\end{figure*}

\begin{figure*}[htb!]
    \centering
    \subfigure[Training loss.]
    {
        \includegraphics[width=0.32\textwidth]{images/DynamicsExperiments/train_loss_cifar}
        \label{fig:trainloss_neural_dynamics}
    }
    \subfigure[Test loss]
    {
        \includegraphics[width=0.32\textwidth]{images/DynamicsExperiments/test_loss_cifar}
        \label{fig:testloss_neural_dynamincs}
    }
    \subfigure[Projections]
    {
        \includegraphics[width=0.32\textwidth]{images/DynamicsExperiments/eigs_cifar_all}
        \label{fig:train_projections_loss_neural_dynamics}
    }
    \caption{Dynamics of neural embeddings where we stop early training the neural kernel and then use the induced representations at the early steps (epochs) to train (as a kernel) the final model. We observe that for a fairly small number of epochs (up to $5,000$) we obtain very sophisticated neural embeddings, as also verified by the overlap measure in Eq. \ref{eq:overlap_measure} (demonstrated in Figure \ref{fig:train_projections_loss_neural_dynamics}).}
    \label{fig:neural_kernel_dynamics}
    %\vspace{-2mm}
\end{figure*}

In addition to the theoretical upper bound, we measure the test error for the studied datasets. Figures \ref{fig:testloss_cifar} and  \ref{fig:testacc_cifar} show respectively the test error and the test accuracy at different steps of the optimization by Gradient Descent for CIFAR-10. We observe that the kernel methods yield significant improvements of both the test error and the accuracy on the test dataset. We observe that the larger the kernel, the larger the improvement. Additionally, we can see a sharper reduction in test error compared to the no-kernel case. This sharp transition (after a small number of steps) is particularly interesting. Because, along such a transition, we observe a significant improvement in the accuracy on test dataset. Thus early-stopping that is commonly used in deep learning can be even more efficient when using kernel methods. 
\\
Finally, similar to the no-kernel case in \cite{Arora19}, by comparing the plots in Figures \ref{fig:train_loss_cifar}, \ref{fig:train_projections_loss_cifar} and \ref{fig:testloss_cifar} we find tight connections between, i) (training) optimization, ii) projection on the top eigenvalues, and iii) generalization. We can therefore improve both training and generalization with kernels since we can get better alignment of the eigenvectors belonging the largest eigenvalues and the target labels.


%\todo[inline]{Update section to only be about CIFAR and fix references}
%In addition to the theoretical upper bound, we measure the experimental test error for each of the datasets. Figure \ref{fig:t} shows the test error at different steps of the optimization by Gradient Descent. We observe, i) on both datasets, the kernel methods yields significantly sharper reduction in error compared to the no-kernel case. This sharp transition (after s small number of steps) is particularly interesting and important. Because, along such a transition, we observe a significant improvement in the accuracy on test datasets, as shown in Figures \ref{fig:test_accuracy} respectively for MNIST and CIFAR-10 datasets. Thus early-stopping that is commonly used in deep learning can be even more efficient when using kernel methods. ii) In long-term and after a large number of optimization steps, the different methods (with or without kernel) perform similarly. However, some of the kernel-based methods perform still (slightly) better in this setting, in terms of both test error (Figure \ref{fig:test_loss}) and test accuracy (\ref{fig:test_accuracy}). \todo{Large kernels are quite a bit better}

%Finally, by comparing the plots in Figures \ref{fig:train_loss}, \ref{fig:train_projections}, \ref{fig:test_loss} and \ref{fig:test_accuracy} we conclude that when using kernels we observe direct relations between (training) optimization, projection on top eigenvalues and generalization, similar to the no-kernel case study in \cite{Arora19}. On the other hand, as discussed, kernels can improve each of them significantly. 

\begin{table}[ht!]
    \centering
     \caption{Accuracy on MNIST test set after n epochs. This dataset is an easy data which after only a small number of epochs, the test error becomes negligible. }
    \begin{tabular}{l | c c c c c c}
\toprule
         $dim(\mathcal{K})$ & \multicolumn{4}{c}{Steps} \\
        &10 &1000 &50000 &100000 \\
    \midrule
    None &0.998582&        0.999527&             0.999527&        0.999527\\
    500 &       0.996690&        0.999054&               0.999054&       0.998582 \\
     1000 &         0.998109 &         0.999054 &        0.999527 &   0.999054 \\
        3072 &         0.998582 &     0.999527 &         0.999527 &     0.999527 \\
        10000 &         0.998582 &         0.999527 &         0.999527 &    0.999527 \\
        
\bottomrule
    \end{tabular}
    \label{tab:testacc_mnist}
\end{table}

\subsection{Neural embedding}
Choosing a proper kernel and its parameters can be challenging \cite{vonLuxburg2007}, as also seen in Table \ref{tab:yHy}. Thus, we investigate a data-dependent neural kernel and embedding. 
For this purpose, we add a second hidden layer to the neural network with $m=10000$ hidden units and ReLU activation. We pre-train this embedding using two different approaches.  The first layer is then kept fix as an embedding where the rest of the network is reinitialized and trained. The first approach is to split the training data in half. We use the first subset to pre-train this three-layer network and the second subset to use for our optimization experiments. In this approach we double $\eta$ to keep the step length the same. The other approach is to use data from a different domain for pre-training. For instance, we use the last two classes of the CIFAR-10 dataset for pre-training the embedding. We compare our results with not using any kernel and with using a RFF kernel with embedding of size 10000.

\subsubsection{Optimization}
Figure \ref{fig:trainloss_neural} shows the training loss for the CIFAR-10 dataset. We observe the neural embeddings achieve faster convergence compared to the previous methods. We report the training loss for neural embedding (same label) on the second (unused) subset of the data, whereas in the other cases we report the results on the full training data. If we use only the second subset for the other methods, we observe very consistent results to Figure \ref{fig:neural_kernel}. 
Figure \ref{fig:train_projections_loss_neural} demonstrates eigenvector projections on the target labels. This shows that both variants of neural embeddings improve alignment of the labels to eigenvectors corresponding to larger eigenvalues (compared to the best RFF kernel). While the effect is unsurprisingly larger when pre-training on the same labels, it is still significantly better when pre-trained on other labels.

\subsubsection{Generalization}
In Figure \ref{fig:testloss_neural} we report the test error on the CIFAR-10. This shows that the neural embeddings perform at least comparable with the best studied RFF kernel. If the  pre-training is done on the same labels we obtain a clear improvement, even if the actual training is only done on a dataset with half the size.

\subsubsection{Dynamics of neural embeddings}
In the previous study, to obtain the neural embeddings (i.e., the pre-trained model), we ran the
neural network for a large number of epochs (i.e., $50,000$), which is computationally inefficient. Here we study the dynamics of neural embeddings and investigate what happens if we stop early training this kernel and then use the induced representations at the early steps to train (as a kernel) the final model. 

The respective results are illustrated in Figure \ref{fig:neural_kernel_dynamics}, which show that
 at the first steps of learning the neural kernel,  the optimization and generalization for the final model improves gradually as we increase the number of steps (epochs). However, after $5000$ epochs of pre-training the kernel, we see that the generalization and optimization of the final model becomes almost stable  and invariant. These results are also consistent with the projections of true labels on eigenvectors of the respective Gram matrices (Figure \ref{fig:train_projections_loss_neural_dynamics}). 
 Our results show that the training process improves the alignment of the eigenvectors of the Gram matrix to the labels and that this reaches close to optimal alignment within the early epochs.
 \subsection{Embeddings with optimized kernels}

So far, we have used two embedding methods: i) a fixed  embedding according to Gaussian kernels, and ii)  the embeddings induced by deep neural networks. In this section we analyze the use of optimal kernels designed for our task of interest. In particular, we study two types of kernels: i) the arc-cosine kernel proposed in \cite{CS09} which optimally represents neural network layers. Note that, as we will discuss, computing this kernel is significantly faster than training a neural network layer. Thus, it can be used for the same purpose, i.e., an optimal embedding induced by a neural network, but in a more efficient way. ii) The model-free kernel learning method proposed in \cite{CortesMohri2012}. Given the training data and the corresponding labels, this method computes the optimal feasible kernel, independent of any classification model or algorithm.

In both cases, we first approximate the kernel embedding using the Nystr\"{o}m method \cite{Nystroem}, and then feed the approximated kernel embedding to the two-layer neural network model, instead of the original data features.

 \begin{figure*}[ht!]
    \centering
    %\hspace{-2mm}
    \subfigure[Training loss.]
    {
        \includegraphics[width=0.32\textwidth]{images/arc-cosine-kernel/train_loss_cifar}
        \label{fig:trainloss_arccosine}
    }
    \hspace{-7mm}
    \subfigure[Test loss]
    {
        \includegraphics[width=0.32\textwidth]{images/arc-cosine-kernel/test_loss_cifar}
        \label{fig:testloss_arccosine}
    }
    \hspace{-7mm}
    \subfigure[Projections]
    {
        \includegraphics[width=0.32\textwidth]{images/arc-cosine-kernel/eigs_cifar_all}
        \label{fig:train_projections_loss_arccosine}
    }
    \caption{The results of the embeddings induced by the arc-cosine kernel with different dimensionality of parameterizations. This kernel  performs better than the Gaussian kernel for sufficiently large number of components and the case where we use the original features as in \cite{Arora19}. The overlap measure in Eq. \ref{eq:overlap_measure} is verified for this case as well.}
    \label{fig:arccosine_kernel}
    %\vspace{-2mm}
\end{figure*}

\begin{figure*}[th!]
    \centering
    %\hspace{-2mm}
    \subfigure[Training loss.]
    {
        \includegraphics[width=0.32\textwidth]{images/alignf/train_loss_cifar}
        \label{fig:trainloss_alignf}
    }
    \hspace{-7mm}
    \subfigure[Test loss]
    {
        \includegraphics[width=0.32\textwidth]{images/alignf/test_loss_cifar}
        \label{fig:testloss_alignf}
    }
    \hspace{-7mm}
    \subfigure[Projections]
    {
        \includegraphics[width=0.32\textwidth]{images/alignf/eigs_cifar_all}
        \label{fig:train_projections_loss_alignf}
    }
    \caption{The results of the embeddings induced by the \emph{alignf} kernel with different dimensionality of parameterizations. This model-free kernel is optimally learned w.r.t. the data and significantly performs better than the arc-cos kernel, the Gaussian kernel and the no-kernel case. We again observe the consistency of a fast optimization, a low test error and a large overlap measure defined in Eq. \ref{eq:overlap_measure}.}
    \label{fig:alignf_kernel}
    %\vspace{-2mm}
\end{figure*}


\subsubsection{Arc-cosine kernel}
The arc-cosine kernel \cite{CS09} mimics the computations in a neural network within an infinite dimensional feature space, where the kernel function is equivalent to the inner product of the feature vectors from a neural network. Then, the Nystr\"{o}m method with different number of components can be used to approximate the kernel embeddings. 
 
The $n$-th order \emph{arc--cosine} kernel between two inputs $x$ and $y$ is computed by
 
\begin{equation}
 k_n(x,y) = \frac{1}{\pi} \|x\|^n \|y\|^n J_n(\theta).
\end{equation}

Where the function $J_n$ and $\theta$ are given by

\begin{equation}
 J_n(\theta) = (-1)^n(sin\theta)^{2n+1}{(\frac{1}{sin\theta}\frac{\partial}{\partial\theta})}^n(\frac{\pi-\theta}{sin\theta})
\end{equation}

\begin{equation}
\theta = cos^{-1}(\frac{x.y}{\|x\| \|y\|})
\end{equation}

In \cite{CS09} it is shown that the computations in single-layer threshold networks is closely related to this kernel. Specifically, the kernel is equivalent to the inner product of embeddings induced by a single-layer threshold network.
Moreover, \cite{CS09} suggests a family of kernels mimicking multi-layer networks based on the base kernel. In our experiments we use the base kernel with $n=0$.

Figure \ref{fig:arccosine_kernel} shows the results of the arc-cosine kernel embeddings. We observe that this kernel (with a sufficiently large number of components) outperforms the Gaussian kernels, and as well as the no-kernel case. Similar to the Gaussian kernel increasing the number of components improves the estimations, and hence, leads to a faster optimization and a lower test error. Moreover, the overlap parameters are also better for  arc-cosine kernel with a large number of compoenents (i.e., arccos 10000). These results show that assuming the arccosine kernel does approximate neural embeddings, then the results of \cite{Arora19} extend to multilayer networks.

 Notice that Neural Tangent Kernel (NTK) \cite{JFH18} is another  approach to compute a kernel representing a neural network. However, the applicability of this method is confined by its very inefficient computational runtime.\footnote{In our experiments on even a significantly smaller dataset (i.e., with only $1000$ images) it took about 24 hours to run the algorithm on GPU.}
 


\begin{figure*}[!t]
    \centering
    %\hspace{-2mm}
    \subfigure[Training loss.]
    {
        \includegraphics[width=0.32\textwidth]{images/Kernel_Learning/train_loss_cifar}
        \label{fig:trainloss_bestkernel}
    }
    \hspace{-7mm}
    \subfigure[Test loss]
    {
        \includegraphics[width=0.32\textwidth]{images/Kernel_Learning/test_loss_cifar}
        \label{fig:testloss_bestkernel}
    }
    \hspace{-7mm}
    \subfigure[Projections]
    {
        \includegraphics[width=0.32\textwidth]{images/Kernel_Learning/eigs_cifar_all}
        \label{fig:train_projections_bestkernel}
    }
    \caption{The consistency of fast optimization, low test error and high overlap between the labels vector and the top eigenvectors. Moreover, we observe a consistent ranking of different kernel methods where \emph{alignf} yields the best results for all the three criteria. The second best method is the arc-cos kernel, followed by the Gaussian kernel. All the three kernels (alignf, arc-cos and Gaussian) outperform the base setting used in \cite{Arora19}.
    }
    \label{fig:bestkernel}
    %\vspace{-2mm}
\end{figure*}
 

\subsubsection{Model-free kernel learning}
Finally, we investigate learning an appropriate kernel, independent of the model or the algorithm to be used for training and classification. For this purpose, we use the method proposed in \cite{CortesMohri2012} that suggests an algorithm to learn a new kernel from a group of kernels based on a similarity measure between the kernels, namely centered alignment. Then, the problem of learning a kernel with a maximum  alignment between the data and the labels is formulated as a quadratic programming (QP) problem. The respective algorithm is called \emph{alignf} \cite{CortesMohri2012}. 

As mentioned, the kernel learning algorithm works based on \emph{centered kernel alignment}. If $K_1$ and $K_2$ are two kernel matrices, the centered alignment between them can be  computed by the following \cite{Gonen2011}.

\begin{equation}
 CA(K_1,K_2) = \frac{\langle K_1^c,K_2^c\rangle_F}{\sqrt{\langle K_1^c,K_1^c\rangle_F\langle K_2^c,K_2^c\rangle_F}} ,
\end{equation}

where $K^c$ is the centered version of the kernel matrix $K$. To find the optimal combination of the kernels (i.e. a weighted combination of some base kernels), \cite{CortesMohri2012} suggests the objective function to be centered alignment between the combination of the kernels and $yy^T$, where $y$ is the labels vector. By restricting the weights to be non-negative, a QP can be obtained as

\begin{equation}
 minimize\hspace{4px} v^TMv - 2v^Ta \hspace{4px}
 w.r.t.\hspace{2px} v \in R_+^P
\end{equation}

 $P$ is the number of the base kernels and $M_{kl} = \langle K_k^c,K_l^c\rangle_F$ for $k,l \in [1,P]$, and finally $a$ is a vector wherein $a_i = \langle K_i^c,yy^T\rangle_F$ for $i \in [1,P]$. If $v^*$ is the solution of the QP, then the vector of kernel weights is given by \cite{CortesMohri2012,Gonen2011}

\begin{equation}
\mu^* = v^*/\|v^*\|
\end{equation}

Figure \ref{fig:alignf_kernel} shows the results of the \emph{alignf} embeddings with different dimensions. We use $7$ Gaussian kernels as the base kernels. This universally optimal method outperforms the other alternatives even the arc-cosine kernel designed as a proxy for neural embeddings. Similar to the previous cases, we observe direct relations between a faster optimization, a better generalization and an improved overlap measure. 

\subsection{Discussion}
We have studied several  kernel embeddings to obtain more sophisticated features for the basic neural network model. 
In Figure \ref{fig:bestkernel} we compare the different kernels with the largest number of dimensions (i.e., when the number of features/components is $10,000$) which provides the most precise approximations.
We observe the consistency of fast optimization, low test error and high overlap between the labels vector and the top eigenvectors. In addition, we observe a consistent ranking of different kernel methods. The model-free kernel learning method in \cite{CortesMohri2012}  (called \emph{alignf}) yields the best results for all the three criteria. The reason could be that it discards the effect of any classification model and learns the universally optimal features. Specifically, the learned kernel is supposed to align well with the label vector, and therefore it results in a better performance in terms of optimization and generalization. 
Then, the second best method is the arc-cos kernel. It mimics the neural embeddings and thus is more suitable than the a priori fixed Gaussian kernel (the kernel embeddings computed directly from a neural network are comparable to the arc-cos kernels, however they require a significantly larger runtime to be computed). Using the original data features yields the worst results, which indicates the importance of proper feature learning and inference for the task of interest.  

Finally, in Table \ref{tab:yHyCompareAll} we compare the theoretical lower bounds on the generalization errors of the different kernels. We observe a consistent ranking with the previous results. The \emph{alignf} method yields the best performance, and the arc-cos and the Gaussian kernels are the next choices. The no-kernel case gives the highest lower bound.

\begin{table}[th!]
    %\vspace{-2mm}
    \centering
    \caption{Quantification of $\mathbf y^T(\mathbf H^\infty)^{-1}\mathbf y$ (or $\mathbf y^T(\mathbf H(\mathcal{K})^\infty)^{-1}\mathbf y$) for different kernels on CIFAR-10 dataset. The alignf method yields the smallest lower bound in the generalization performance.}
    \begin{tabular}{l l r}
    
    \toprule
    Kernel & Dimension  & CIFAR-10 \\
          \midrule
          Gaussian & 10000 & 44630 \\
          arc-cosine & 10000 & 33698\\
          alignf & 10000 & 10618 \\
          \multicolumn{2}{l}{No kernel} & 74670\\
        \bottomrule
    \end{tabular}
    \label{tab:yHyCompareAll}
    %\vspace{-5mm}
\end{table}

==> old-intro.tex <==
\iffalse
Deep neural network models \cite{BengioCV13,LeCunBH15,Schmidhuber15} provide the state-of-art results in several tasks and applications, although the theory has not been completely understood yet.
The well-known work of \cite{Zhang17} highlighted intriguing experimental phenomena about deep network training -- specifically, optimization and generalization -- and called for a rethinking of generalization in statistical learning theory. In particular, two fundamental questions that need understanding are:
\\

{\bf Optimization.} Why do true labels give faster convergence rate than random labels for gradient descent?
\\

{\bf Generalization.} What property of properly labeled data controls generalization?
\\

\cite{Arora19} have recently tried to answer this question in a simple two--layer model by conducting a spectral analysis of the associated Gram matrix. They show that both training and generalization are better if the label vector aligns with the top eigenvectors. 

However, their analysis applies only to a simple two layer network. \emph{How could their insights be extended to deeper networks? }

A widely held intuitive view is that deep layers generate expressive \emph{representations} of the raw input data. Adopting this view, one may consider a model where a representation generated by successive neural network layers is viewed as a \emph{kernel embedding} which is then fed into the two--layer model of \cite{Arora19}. The connection between neural networks and kernel machines has long been studied; \cite{CS09} introduced kernels that mimic deep networks and \cite{TKG18} showed kernels equivalent to certain feed--forward neural networks. Recently, \cite{Belkin18} also make the case that progress on understanding deep learning is unlikely to move forward until similar phenomena in classical kernel machines are recognized and understood. 
%Very recently, \cite{JFH18} showed that the evolution of a neural network during training can be related to a new kernel,  the Neural Tangent Kernel (NTK) which is central to describe the generalization properties of the network.
%Here we pursue this approach by studying the effect of incorporating embeddings into the simple two layer model and we perform a spectral analysis of these embeddings along the lines of \cite{Arora19}. 

The fundamental question we address is: \emph{Do representations provided by  kernel embeddings help in training and generalization}? We address this question in the context of the simple model of \cite{Arora19} and their approach based on a spectral analysis of the associated Gram matrix. Specifically, we take a view of a multi--layer network as first producing an embedding $\phi(x)$ of the input which is then fed as input to the simple two layer network of \cite{Arora19}. While a general transformation $g(x)$ of the input data may have arbitrary effects, one might expect a universal kernel representation to improve performance. Do kernel representations create a better alignment of labels with the top eigenvectors of the Gram matrix? We investigate this first by using an unbiased kernel such as Gaussian kernel, using random Fourier features(RFF) to approximate the Gaussian kernel embedding \cite{RR07}.

Next, we address the question: \emph{Do representations provided by neural embeddings help in training and generalization?} We address this in two ways: first, we use kernels that have been designed to specifically mimic neural networks \cite{CS09}. Then we use data driven embeddings explicitly produced by the hidden layers in neural networks:  either using a subset of the same training data to compute such an embedding, or transfer the inferred embedding from a different (but similar) domain. 
%Once again we observe substantial improvements in both training and generalization.
%\begin{itemize}
%\textbf{i.} We can use an unbiased kernel such as Gaussian kernel. This choice is consistent with the maximum entropy principle and makes no prior assumption about the data. Or use a kernel which mimics or approximates deep networks\\
%\textbf{ii.} We could use data driven embeddings explicitly produced by the hidden layers in neural networks:  either use a subset of the same training data to compute such an embedding, or transfer the inferred embedding from a different (but similar) domain. 
%\end{itemize}

%While a general transformation $g(x)$ of the input data may have arbitrary effects, one would expect kernel and neural representations to improve performance. 
 %We address the aforementioned two fundamental questions in the setting where we employ a kernel representation of the input, for example, the Gaussian kernel. 
%Kernel methods are one of the pillars of machine learning, as they give us a flexible framework to model complex functional relationships in a principled way and also come with well-established statistical properties and theoretical guarantees.
%{\bf Optimization.}  
%{\bf Generalization.} We also achieve significantly lower test error and we confirm that the data dependent spectral measure introduced in \cite{Arora19} significantly improves with kernel and neural embeddings.

We indeed find substantial improvements in both training and generalization using any of the above kernel representations.

Finally we ask the question: \emph{What is the optimal representation for optimization and generalization?} The work of \cite{Arora19} suggests seeking a representation which makes the label vector align best to the top eigenvectors of the associated Gram matrix. This connects to the problem of \emph{kernel--target alignment} \cite{Christ01,CortesMohri2012}. We use the criterion suggested in these papers as a proxy for aligning the label vector to the top eigenvectors and compute the representation so produced. Indeed we observe that this representation provides the best results for training and generalization.

Thus this work shows that kernel and neural embeddings improve the alignment of target labels to the eigenvectors of the Gram matrix and thus help training and generalization. This suggests a way to extend the insights of \cite{Arora19} to deeper networks, and possible theoretical results in this direction.
%In addition to throwing further light on the analysis in \cite{Arora19}, our results also support and confirm the widely held view that representations play a key role in both optimization and generalization in deep learning models. 
%Much past work has been done to investigate the equivalent kernel of certain neural networks, either experimentally (Burgess, 1997), through sampling (Sinha \& Duchi, 2016; Livni et al., 2017; Lee et al., 2017), or analytically by assuming some random distribution over the weight parameters in the network (Williams, 1997; Cho \& Saul, 2009; Pandey \& Dukkipati, 2014a;b; Daniely et al., 2016; Bach, 2017a).\todo{Make sure to decide /fix references. Add tushida} 

%{\bf Neural embeddings.}
%Choosing a proper kernel and setting its parameters can be challenging \cite{vonLuxburg2007}, in particular with an unbiased kernel such as Gaussian kernel. This choice is consistent to the maximum entropy principle and makes no prior assumption about the data. Therefore, in the second approach, we perform a data-dependent spectral analysis instead.  
%We investigate experimentally the effect of representations produced by the hidden layers in neural networks and show that indeed they offer benefits to training and generalization even more than those from data-agnostic Gaussian kernel embeddings. We perform the data-dependent neural embedding in two ways. We  either use a subset of the same training data to compute such an embedding, or, we transfer the embedding inferred from a different (but similar) domain. 


%Although we have used explit embeddings at the input layer, our analysis suggests that the same beneficial effects might obtain with the representations learned by deep learning models.
\fi


We extended the recent results of \cite{Arora19} by a spectral analysis of the representations corresponding to different kernel and neural embeddings and showed that such representations benefit both optimization and generalization.
We demonstrated the applicability of the overlap criteria in \cite{Arora19} for analysing the impacts of different kernels. 
In particular, we showed that learning a model-free kernel yields the best results in terms of fast optimization, low generalization error, and large overlap between the top  eigenvectors and the labels vector. 
By combining recent results connecting kernel embeddings to neural networks such as \cite{TKG18}, one may be able to extend the fine--grained theoretical results of \cite{Arora19} for two layer networks to deeper networks.

==> rebut.tex <==
1. The differences between this paper and [Phuong and Lampert, 2019] is not clear. Thus, please provide more analysis to make it more clear.

As we discuss in section  2.1, [Phuong and Lampert, 2019] consider only a deep 'linear' network and heavily use convexity arguments.


2. The authors use CIFAR-10 for experiments in Section 5, and only look at the first two classes. However, why not use all classes of CIFAR-10?

We study knowledge distillation consistent to the kernel regime setting in [Arora et al 2019] and other works where they perform the numerical studies with the first two classes. We argue that our results hold for other number of classes as well. 

3. In Section 5.3, experimental results on the two-layer model demonstrate the effectiveness of the kernel embedding. However, the effect of the kernelembedding on popular networks, such as ResNet [1] and MobileNetV2 [2], is unclear. Thus, please provide more results on it. 

The kernel regime is the most common stetting that the prior work considers to study the theory of deep learning [Arora et al., 2019,Du and Hu, 2019,Cao and Gu, 2019]. We leave the extension to deeper networks to future work (Ashkan, can we say more here?)

4. The authors propose the theoretical analysis of knowledge distillation (KD) to help us understand KD. To some extent, is it able to further help us improve the KD mechanism or framework?

Indeed our analysis offers several practical insights for better knowledge distillation: (1) the right balance between the use of original data and "dark knowledge" of the teacher (2) size of the intermediate teacher (section 3.2) (3) the use of better representations in the teacher (5.2, 5.3).

1. The theoretical novelty is very limited. For generalized KD setting, the only difference to Arora et al., 2019, is the training objective. Therefore, most of the analysis can be borrowed or developed from the results in Arora et al., 2019 with minimal effort.

As we stress in the introduction, the dynamics of the regularized optimization introduces significant new difficulties. To address these we need to introduce several new tools and techniques that "go significantly beyond the previous literature".

2. The theoretical results mainly concern the training error of the student network. However, for KD, the central question should be why does KD canimprove the generalization performance

Our results focus on the analysis of the training dynamics but has implications for generalization: the dynmics limits the class of weights and in this way translates into generalization results in the standard way via Rademacher complexity techniques as in [Arora et al 2019].



==> related.tex <==
In its current and most widely known form, distillation was introduced by Hinton et al. \cite{hinton15} with the aim of compressing neural networks. Since then, distillation has quickly gained popularity among practitioners and established its place in deep learning folklore with a wide range of applications.

%In contrast to its empirical success, a rigorous theoretical understanding of the principles underlying the effectiveness of distillation have largely remained a mystery. 
Until recently, Lopez-Paz et al. \cite{LopezPaz15} was the only work that tried to examine distillation from a theoretical perspective. It casts distillation as a form of Vapnik's notion of learning using privileged information, a learning setting in which additional per-instance information is available at training time but not at test time. Their paper is more a heuristic argument for the effectiveness of distillation with repect to generalization error rather than a rigorous analysis. Very recently, Phuong and Lampert \cite{phuong19} made the first attempt to analyze distillation in a simple model. In their setting, both the teacher and the student are \emph{linear} classifiers (although the student's weight vector is allowed a over-parametrized representation as a product of matrices). They give conditions under which the student's weight vector converges (approximately) to that of the teacher and derive consequences for generalization error. Crucially, their analysis is limited to linear networks while we analyze distillation in the context of non-linear networks.
%
A series of recent papers  e.g. \cite{Arora19,DuH19,CaoG19a} achieved breakthroughs in understanding how (infinitely) wide neural network training behaves in the so-called kernel regime. In this regime, the dynamics of training by gradient descent can be approximated by the dynamics of a linear system. We extend the repertoire of the methods that can be applied in such settings.

==> theory.tex <==
\paragraph{Network model.}
In \cite{Arora19}, the authors consider a simple two layer network model:
\begin{equation}
    f_{\bm W,\bm a}(\bm x) = \frac{1}{\sqrt{m}}\sum_{r=1}^m a_r \max(0, \bm w_r^T \bm x_i), 
\end{equation}
with $\bm x\in \R^d$, $\bm w_1$, .. $\bm w_m \in \R^{d\times m}$ and ($a_1$, .. $ a_m)^T \in \R^m$ (where $m$ specifies the number of neurons in the hidden layer, i.e., its width). These can be written jointly as $\mathbf a=( a_1, ..,  a_m)^T$ and $\mathbf W=(\bm w_1, .. , \bm w_m)$. This network is trained on dataset of data points $\{x_i\}$ and their targets $\{y_i\}$.

They provide a fine grained analysis of training and generalization error by a spectral analysis of the \emph{Gram matrix}:
\begin{equation}
 \mathbf H^{\infty}_{i,j} := E_{\mathbf W\sim \mathcal{N}(0,\bm{\mathcal{I}})}\mathbf x_i^T  \mathbf x_j 1[ \mathbf w^T \mathbf x_i \geq 0, \mathbf w^T \mathbf x_j \geq 0].
\end{equation}
If 
\begin{equation}
    \mathbf H^{\infty}  = \sum_i \lambda_i \mathbf v_i \mathbf v^T_i
\end{equation} 
is the orthonormal decomposition of $\mathbf H^{\infty}$, \cite{Arora19} show that both training and generalization are better if the label vector $y$ aligns with the eigenvectors corresponding to the top eigenvalues of $\mathbf H^{\infty}$. 
\iffalse
particular 
\begin{itemize}
    \todo{Do we not need $\eta$ here?}
    \item $\sum_i (1 - \lambda_i)(v^Ty)^2$ determines the convergence rate of gradient descent training.
    \item $y^T (H^\todo{$\infty$?})^{-1}y = \sum_i \frac{1}{\lambda_i} (v_i^Ty)^2$ determines the generalization error.
\end{itemize}
\fi 

We extend the two-layer ReLU network in \cite{Arora19} via adding different types of embeddings $\phi$ at the input layer corresponding to a kernel $\mathcal{K}$.
The corresponding model is:
\begin{equation}
\label{eq:model}
    f_{\mathbf{W},\mathbf{a}}(\mathbf{x}) = \frac{1}{\sqrt{m}}\sum_{r=1}^m a_r \max(0, \mathbf{w}_r^T \bm{\phi}(\mathbf{x}_i)).
\end{equation}

For a representation $\left(\bm \phi(\bm x_i),i \in [n]\right)$ corresponding to a kernel $\mathcal{K}$, define the Gram Matrix
\begin{equation}
    \mathbf H(\mathcal{K})^{\infty}_{i,j} := E_{\mathbf W}\mathcal{K}(\bm x_i,\bm x_j) 1[ \mathbf w^T \bm \phi(\bm x_i) \geq 0, \mathbf w^T \bm \phi(\bm x_j) \geq 0]
\end{equation} 
and let its eigenvalues be ordered  as 
\begin{equation}
    \lambda_0(\mathcal{K}) \geq \lambda_1(\mathcal{K}) \geq \cdots \geq \lambda_{n-1}(\mathcal{K})
\end{equation} and let $\mathbf v_0(\mathcal{K}),\cdots, \mathbf v_{n-1}(\mathcal{K})$ be the corresponding eigenvectors. 
%Given a labelling $y_i, i\in [n]$, normalize it so that $\sum_i (v^T_i y)^2  = 1$. 

A kernel $\mathcal{K}$ such that the corresponding eigenvectors align well with the labels would be expected to perform well both for training optimization as well as generalization. This is related to kernel target alignment \cite{Christ01}.

\subsection{Optimization}
For the simple two layer network, \cite{Arora19} show that the convergence of gradient descent is controlled by
\begin{equation}
 \sqrt{\sum_i (1 - \eta \lambda_i)^{2k} (\mathbf v_i^T \mathbf y)^2}
\end{equation}
%
For our kernelized network, the corresponding convergence is controlled by
\begin{equation}
 \sqrt{\sum_i (1 - \eta \lambda_i(\mathcal{K}))^{2k} (\mathbf v(\mathcal{K})_i^T \mathbf y)^2}
\end{equation}
%
\\
\subsection{Generalization}
For the simple two layer network, \cite{Arora19} show that the bound on the generalization performance is dominated by 
\begin{equation}
 \mathbf y^T(\mathbf H^\infty)^{-1}\mathbf y
 \label{eq:gen}
\end{equation}
For our kernelized neural network model, the corresponding data \emph{and} representation dependent measure is:

\begin{equation}
 \mathbf y^T(\mathbf H(\mathcal{K})^\infty)^{-1}\mathbf y
 \label{eq:gen_kernel}
\end{equation}

\iffalse
Given two data representations $(\phi,x,y):= (\phi(x_i),y_i), i \in [n]$ and $(\phi',x,y'):= (\phi'(x_i),y'_i), i \in [n]$ (normalized as above) we say that $(\phi,x,y)$ \emph{majorizes} $(\phi',x,y')$, written $(\phi,x,y) \succeq (\phi',x,y')$ \cite{marshall11} if for each $k \in [n]$, 
\[ \sum_{i=1}^k (v_i^T y)^2 \geq \sum_{i=1}^k (v'_i^T y')^2 
\]

\begin{theorem}
Let $(\phi,x,y) \succeq (\phi',x,y')$. Then 
\begin{itemize}
    \item The gradient descent optimization applied to $(\phi,x,y)$ dominates that applied to $(\phi',x,y')$
    \item $y^T (H^{\phi})^{-1} y \leq 
       y'^T (H^{\phi'})^{-1} y'$ and so 
       $(\phi,x,y)$ dominates $(\phi',x,y')$ with respect to generalization error.
\end{itemize}
\end{theorem}
\fi

